Detection of HF and VHF Fields through Floquet Sideband Gaps by `Rabi Matching' Dressed Rydberg Atoms

Radio frequencies in the HF and VHF (3 MHz to 300 MHz) bands are challenging for Rydberg atom-based detection schemes, as resonant detection requires exciting the atoms to extremely high energy states. We demonstrate a method for detecting and measuring radio frequency (RF) carriers in the HF and VHF bands via a controlled Autler-Townes line splitting. Using a resonant, high-frequency (GHz) RF field, the absorption signal from Townes-Merrit sidebands created by a low frequency, non-resonant RF field can be enhanced. Notably, this technique uses a measurement of the optical frequency separation of an avoided crossing to determine the amplitude of a non-resonant, low frequency RF field. This technique also provides frequency-selective measurements of low frequency RF electric fields. To show this, we demonstrate amplitude modulated signal transduction on a low frequency VHF carrier. We further demonstrate reception of multiple tones simultaneously, creating a Rydberg `spectrum analyzer' over the VHF range.

==> texttakenoutofmain.tex <==


% abstract

%We present an experimental method for detecting radio frequency carriers in the HF and VHF (3 to 300~MHz) range via a controlled Autler-Townes line splitting using excited Rydberg atoms. 
%An applied ``Low Frequency'' electric field modulates the Stark energy shift of the Rydberg state, generating quasi-energy sidebands.
%Adding a resonant microwave field and matching the Rabi frequency to the target signal's frequency, we observe an avoided crossing in the spectrum that grows non-linearly with field strength. 
%Using a combined dressed state and Floquet model with effective state polarizabilities, we are able to predict the observed spectral features corresponding to ac amplitude, dc offset, and frequency, but more realistic models and careful experimentation are needed for precise measurements using this technique. 
%Looking toward applications, we demonstrate AM signal transduction on a low-frequency carrier, and compare it to other Rydberg sensing methods.
%We also demonstrate reception of multiple tones simultaneously, creating a Rydberg `spectrum analyzer' over the VHF range, although we also observe additional frequency sum and difference signals. 
% In the course of this investigation, we also realized a modification to a non-resonant Stark-shifting detection method, where the addition of a Rydberg dressing field increases experimental sensitivity by nearly a factor of two. 


% When the HF field is present, AT peak imbalance suggests $\omega_{dr}$ is detuned at low dressing power, but comes into resonance at higher dressing power, suggesting that an additional ac Stark shift due to the dressing field is present. 
% To compensate for this, theory curves use a scaling parameter $S_{\delta}$ microwave detuning to resemble the data more closely. 



% \section{Old Theory - WRONG ? }\label{secThe}
% Much of the atomic and optical theory follows from EIT and dressed-atom formalism that is common in the literature \cite{}. We focus on the splitting of the Rydberg-Rydberg transition as a two-level system, where one atomic state's level structure is read out by two photon EIT for the experiment, as detailed in Section~\ref{secExp}. 

% Consider two atomic states, $\ket{e}$ and $\ket{g}$, `excited' with higher energy than `ground,' that are separated in energy by $E_e-E_g=hf_{eg}=\hbar\omega_{eg}$.
% Applying an oscillating electric field nearly resonant to the transition frequency $f_{eg}$ will drive populations between the states, and adjust the energy of the system, generating the splitting. 
% We can consider the nearly degenerate states $\ket{e}$ and $\ket{g+\hbar\omega}$, where the applied RF frequency $\omega$ is not far from resonance $\omega_{eg}$. 

% The measure of coupling strength is called the Rabi frequency, and is given by $\hbar\Omega_{eg} = E\cdot d_{eg}$, where the state-to-state dipole transition strength is $d_{eg} = \bra{e}e\cdot\textbf{r}\ket{g}$. 
% Notably, Rabi scales linearly with electric field strength, as well as the particular atomic dipole transition strength, which can be as large as 1000's of times $ea_0$ between Rydberg states. 
% As the frequency is scanned across resonance, this Rabi frequency enactes an avoided level crossing, where states' energies remain separated in energy by at least the Rabi frequency. 

% Assembling these components into a Hamiltonian for the two-level $(\ket{e},\ket{g})$ system (ignoring decay and other effects) would be:
% \begin{equation}
% H = 
% \left( \begin{array}{cc}
% 0 & \Omega_{eg}/2 \\
% \Omega^*_{eg}/2 & \delta
% \end{array} \right)
% \end{equation}
% Diagonalizing, our two-level atomic system transforms into a two-level dressed system, with energy gap dependant on detuning $\delta=\omega-\omega_{eg}$ and Rabi as the `generalized Rabi Frequency' $\Omega' = \sqrt{\delta^2+\Omega_{eg}^2}$.
% This represents the observable spectroscopic splitting, smallest on resonance with equal-sized peaks separated by exactly the Rabi frequency, then split further with RF applied off-resonance, with imbalanced spectral line height by way of population from the observed Rydberg state. 

% The dressed states of the system are coherent mixtures of the excited and ground states, where the mixing angle $\theta$ depends on detuning and Rabi frequency.  
% \begin{eqnarray*}
% \ket{+} =& \sin(\theta)\ket{e} + \cos(\theta)\ket{g + 1\gamma} \\
% \ket{-} =& \cos(\theta) \ket{e} - \sin(\theta)\ket{g + 1\gamma}
% \end{eqnarray*}
% where $\cos(\theta) = \frac{\Omega_{eg}}{\sqrt{\Omega_{eg}^2+(\Omega'-\delta)^2}}$ and 
% $\sin(\theta) = \frac{\Omega'-\delta}{\sqrt{\Omega_{eg}^2+(\Omega'-\delta)^2}}$. 
% \textcolor{red}{re-derive this/check it, stole this from Drew's thesis p 53}.
% On resonance, the states are in equal mixture and out of phase:
% \begin{eqnarray*}
% \ket{+} =& \frac{1}{\sqrt{2}}\ket{e} + \frac{1}{\sqrt{2}}\ket{g + 1\gamma} \\
% \ket{-} =& \frac{1}{\sqrt{2}}\ket{e} - \frac{1}{\sqrt{2}}\ket{g + 1\gamma}
% \end{eqnarray*}

% Considering that we now want to dress \textit{these} dressed states, we should consider the Rabi frequency in that system. As before, we can insert the dipole operator(?) $e\cdot\textbf{r}$ between our states: $d_{+-} = \bra{+}e\cdot\textbf{r}\ket{-}$, yielding:
% \begin{eqnarray*}
% d_{+-} = \frac{1}{2} e \times \\
% \left[\bra{e}\textbf{r}\ket{e} - \bra{e}\textbf{r}\ket{g} + \bra{g}\textbf{r}\ket{e} - \bra{g}\textbf{r}\ket{g} \right]
% \end{eqnarray*}
% The first and fourth term represent forbidden (self-same) transitions thus are zero, but the middle terms sum ($\Omega=-\Omega^*$???) to cancel the factor of $\frac{1}{2}$. 
% \textcolor{red}{sign error? included the minus sign, now they cancel? If this Rabi is ``imaginary'' then this is true. ... is this a rotation around iy on the bloch sphere? }
% This result shows that the dressed-dressed dipole strength is that of the Rydberg-Rydberg transition: $d_{+-} = d_{eg}$.
% That is, we get to retain the large dipole moments of the Rydberg states, while implementing a tunable resonance. 

% We can apply the two-level dressed atom approach from earlier in the same manner, but using the $\ket{+}$ and $\ket{-}$ states as the basis, defining each as coherent mixtures of $\ket{e}$ and $\ket{g}$. 
% As briefly mentioned, the EIT probe can observe only one of the Rydberg states, say $\ket{g}$, which has its line split, twice. 
% The state $\ket{g}$ will be split by $\Omega_{eg}$ into two lines $\ket{+}$ and $\ket{-}$, then further each of these lines is split by $\Omega_{+-}$ into four states $\ket{++}$, $\ket{+-}$, $\ket{-+}$, and $\ket{--}$, each containing some fraction of $\ket{g}$ or $\ket{e}$ to be observed spectroscopically. 
% We can expect four equal height peaks if both the splitting power is resonant to the Rydberg-Rydberg transition, and the signal RF is resonant to the Rabi splitting. 


% We also employ a multi-tone generating RF signal, where modulation of a 150~MHz carrier generates equal power, equally-spaced sidebands up to bandwidth 80 MHz. 
% Multi-tone signals show in this work include three tones: \{125,150,175\} and five tones: \{110,130,150,170,190\}.
% We verified the expected operation of the multi-tone generator with a spectrum analyzer, although as we discuss later, we observed tone sidebands at half the expected frequency, which may be a result of the method of generation, as opposed to the power combining of two independently-sourced tones. 


% \begin{figure*}    
%     \centering
%     \begin{overpic}[width=\textwidth]{100MHz_data_with_theory.pdf}
%     \put(51.2,7.7){{\Large $\square$} dc}
%     \put(52.2,10){{\Large $\square$} ac}\end{overpic}
%     \caption{Comparison of experiment and theory. 
%     Top: Observed transmission spectra, with a `waterfall' over dressing field $\Omega_{dr}$ vertically, with each separate plot from left to right increasing the field strength ($\sqrt{P_{HF}}$) of a 100 MHz HF field on the plates. 
%     Bottom: Calculated Quasi-energy spectrum over the dressing $\Omega_{dr}$ waterfall and quasi-energy $\varepsilon$ axes, with marker area corresponding to the state projection of $\ket{56D_{5/2}}$ into the dressing-Floquet eigen-states. 
%     This calculation uses $E_{dc}=0.02$~(V/cm), $N_{max}=24$, $\delta_{dr} = 1.05 \cdot (\langle\Delta_D\rangle - \langle\Delta_F\rangle) $, varying $\Omega_{dr}$ and $E_{HF}$ as labeled.
%     \label{fig:ScanDressing}}
% \end{figure*}


% \begin{figure*}
%     \centering
%     \begin{overpic}[width=0.495\columnwidth]{56ac_LF_scan.pdf}
%     \put(-2,60){(a)} \put(-2,10){(b)} \end{overpic}
%     \begin{overpic}[width=0.495\columnwidth]{100ac_LF_scan.pdf}
%     \put(-2,60){(c)} \put(-2,10){(d)} \end{overpic}
%     \begin{overpic}[width=0.495\columnwidth]{200ac_LF_scan.pdf}
%     \put(-2,60){(e)} \put(-2,10){(f)} \end{overpic}
%     \begin{overpic}[width=0.495\columnwidth]{200dc_LF_scan.pdf}
%     \put(-2,60){(g)} \put(-2,10){(h)} \end{overpic}
%     \caption{Effect of increasing HF field, comparing data with theory. 
%     These plots hold $\Omega_{dr}$ constant, keeping experimental $\delta_{dr}\simeq0$ as $E_{HF}$ grows ($E_{dc}=0.02$~(V/cm)), using $\delta_{dr}=0$ in the theory curves. 
%     We show data using 56~MHz (a,b), 100~MHz (c,d), 200~MHz (e-h), with values of  $\Omega_{dr}$ which demonstrate the ac (a-f), and the dc (g,h) splittings. 
%     \label{fig:scanlowfreq}    }
% \end{figure*}


% Looking toward applications of HF and VHF reception of signals on carriers, we demonstrate the ability to transmit audio-band information by amplitude modulating (AM) the HF carrier. We use a lock-in amplifier of the EIT transmission during $\delta_C$ scans, referenced to the AM signal, choosing the `$R$' or amplitude component of a lock-in signal as the phase changes across input parameters. This allows for easy optimization of $\Omega_{dr}$ and $\omega_{dr}$ as we vary $\omega_{HF}$. 
% We amplitude modulate $E_{HF}$ at 10~kHz, with depth 50\%, and use $P_{HF}=-10$~dBm ($\approx0.14$~(V/cm) at 100~MHz) for all cases, comparing lock-in sensitivities using different powers of $\Omega_{dr}$. 
% This data does not include the $\ket{56D_{3/2}}$ peak, and does not have a frequency reference other than the HF features. 

% First, we examine the shifting of the center EIT peak due to only the HF field's Stark shifts \cite{liu2022highly}. 
% The AM shifts the center EIT line back-and-forth as the time-averaged shift ($\Sigma_D^\sim$) is modulated, generating two lock-in sensitivity peaks at the highest slopes on either side of the center line, measured in Fig.~\ref{fig:signals}(a). 
% Given the quadratic nature of this shift, we would expect sensitivity to improve with base HF power, or the addition of a DC field \cite{meyer2021waveguide}.
% This method yields a significant signal, but must compete with the entire spectrum of electric fields that similarly shift the center line. 

% Second, we add a weak dressing field to partially split the line to an optimally sensitive slightly split configuration as seen in Fig.~\ref{fig:signals}(b). 
% As the HF field's stark shifts modulate the Rydberg energy levels, $\delta_{dr}$ is effectively frequency modulated (FM) against the constant $\omega_{dr}$.
% Looking at the AT dressed states, their populations are balanced when $\omega_{dr}$ is resonant to the Stark-shifted states, but vary with detuning, shifting population back-and-forth between the dressed states, changing peak heights, as the AM brings $\omega_{dr}$ above and below resonance. 
% We find this scheme improves sensitivity by roughly a factor of two.


% The first Stark shifting method's sensitivity is determined by the transmission edge slopes, whereas this second `FM' depends on the AT peak heights and relation between $\delta_{dr}$ and $\Omega_{dr}$. 
% Both modulated signals are shown with their respective lock-in signals in Fig.~\ref{fig:signals}(a,b).
% This `FM' scheme using a small dressing field remains broadband, and effectively measures a Stark shift from any frequency source for the same reasons as the first method. 

% Third, using the method in this letter, we use strong dressing field power to observe the avoided crossing at the center of this work, shown in Fig.~\ref{fig:signals}(c).
% This measurement is conceptually similar to AM detection with Rydberg atoms using a resonant microwave, where a line's splitting is modulated, giving highest sensitivity between the peaks when they are one linewidth apart. 
% We expect this method will have a sensitivity which depends on $E_{HF}$ amplitude, and we plan to examine sensitivity and bandwidth of this technique further. 
% We find optimized lock-in signals when the Rabi frequency $\Omega_{dr}$ is `matched' to $\omega_{HF}$ and $2\omega_{HF}$, where we are able to `resonantly' detect amplitude changes of the HF field.
% In effect, only certain portions of the population are brought to resonance when  $\Omega_{dr}\approx\omega_{HF}$ or $2\omega_{HF}$ locally, due to the non-uniformity of the dressing field. 
% The spread of $\Omega_{dr}$ values gives the approximate bandwidth of this  spectral `band-pass'.  
% Generally, the $\pm2$ features are more sensitive than the $\pm1$ features, (as $E_{HF}^2$ over linear $E_{HF}$), although this competes with the broadening from the higher $\Omega_{dr}$ fields needed to measure the $\pm2$ features compared to the $\pm1$ pair.
% We find this method has comparable sensitivity, but broadening of the AT peaks decreases sensitivity at higher $\omega_{HF}$ frequencies. This may be dues to field non-uniformity for higher frequencies, which is a technical limitation that can be overcome.

% To illustrate signal fidelity, we send music through the atoms, showing the modulation signal and resulting transmission for transduction in Fig.~\ref{fig:signals}(e), using a 100~MHz carrier, with optimized $\Omega_{dr}$ coupling laser $\delta_C$ locked near the lock-in peak location. 
% old caption: 
% \begin{overpic}[width=\columnwidth]{fig5abcd.pdf}
    % \put(40,47){(a)} \put(40,30){(b)} \put(40,14){(c)} \put(90,45){(d)} \end{overpic}
    % % \begin{overpic}[width=\columnwidth]{one_audio.pdf}
    % % \put(91,47){(e)}\end{overpic}
    % \begin{overpic}[width=\columnwidth]{fig5e.pdf}
    % \put(91,27){(e)}\end{overpic}
%  \caption{Comparison of audio signal transduction techniques.
%     Spectra and corresponding lock-in ($R$) signal for an amplitude-modulated 150~MHz carrier, showing sensitivity to AM signals for three schemes: 
%     (a) HF signal only, 
%     (b) HF with a slight dressing field, and
%     (c) using a resonant $\Omega_{dr}$, per this paper. 
%     The highest peak of each lock-in trace (10 kHz, 50\% AM) across tested frequencies are plotted in (d).  
%     (e) Example of music as the am signal on a 100~MHz carrier.
%     We show the AM voltage signal (black) and the received photo diode voltage (magenta).
%     }



% By comparison of theory and experimental data from Sec.~\ref{sec:Res}, we obtain background dc electric field $E_{DC} \approx 0.02$~V/cm, and a power-to-field conversion factor of $0.40$~V/cm per $\sqrt{\textrm{mW}}$, or $\sim0.16$~(V/cm)$^2$ per mW of HF power $P_{HF}$ applied at 100~MHz on the plates.
% We estimate the error in these measurements at roughly $10\%$, for fits done `by eye,' as we have yet to develop a rigorous fitting procedure for the data. 
% The uncertainty in HF electric field measurement is dominated by theory calculations of a Rydberg state's effective polarizability, and experimentally by the broadening of AT lines due to reflections from the dowels and other elements.

  % \cite{rotunno2022modeling}. 
% Comparing theory and experiment yields $0.44$~V/cm per $\sqrt{\textrm{mW}}$, or $\sim0.2$~(V/cm)$^2$ per mW of $P_{HF}$ applied at 100~MHz in this external plate structure, whose uncertainty is dominated by calculated state polarizabilities and the line-broadening due to spatial variations in $\Omega_{dr}$.


% \cite{latypov2022compact}.
%There have been many previous attempts at `state tuning' which can cause far off-resonant HF fields to be detected.
%Off-resonant AT or `generalized' Rabi frequency measurements using ac Stark shifts are possible nearby existing resonances \cite{simons2016using}, or farther away with a strong local oscillator (LO) \cite{hu2022continuously}. % we can talk about this ac stark def 
%When using dc Stark shifts to measure intensity, a major gain in sensitivity is added with a strong dc field, biasing the quadratic Stark shift, and further an LO can tune the reception band using a vacuum waveguide, demonstrated from dc to 20 GHz \cite{meyer2021waveguide}.

% With laser frequencies fixed, this EIT-AT method also enables reception of AM and FM signals on carriers \cite{meyer2018digital, anderson2020atomic, holloway2020multiple, zou2020atomic, fancher2021rydberg, liu2022deep, meyer2022simultaneous, prajapati2022tv, borowka2022sensitivity, meyer2022simultaneous}, notably without the need for down-conversion to read out the signal modulation.
% An rf LO is used to improve sensitivity of measurements with a heterodyne technique \cite{gordon2019weak, hao2020precise, jing2020atomic, jia2021span, cai2022sensitivity}, as well as providing a phase reference for angle-of-arrival measurements \cite{simons2019rydberg, robinson2021determining}, and enabling phase shift keying communication protocols \cite{holloway2019detecting}.







